Hypersequent Calculi Have Ackermannian Complexity

For substructural logics with contraction or weakening admitting cut-free sequent calculi, proof search was analyzed using well-quasi-orders on $\mathbb{N}^d$ (Dickson's lemma), yielding Ackermannian upper bounds via controlled bad-sequence arguments. For hypersequent calculi, that argument lifted the ordering to the powerset, since a hypersequent is a (multi)set of sequents. This induces a jump from Ackermannian to hyper-Ackermannian complexity in the fast-growing hierarchy, suggesting that cut-free hypersequent calculi for extensions of the commutative Full Lambek calculus with contraction or weakening ($\mathbf{FL_{ec}}$/$\mathbf{FL_{ew}}$) inherently entail hyper-Ackermannian upper bounds. We show that this intuition does not hold: every extension of $\mathbf{FL_{ec}}$ and $\mathbf{FL_{ew}}$ admitting a cut-free hypersequent calculus has an Ackermannian upper bound on provability. To avoid the powerset, we exploit novel dependencies between individual sequents within any hypersequent in backward proof search. The weakening case, in particular, introduces a Karp-Miller style acceleration, and it improves the upper bound for the fundamental fuzzy logic $\mathbf{MTL}$. Our Ackermannian upper bound is optimal for the contraction case (realized by the logic $\mathbf{FL_{ec}}$).

==> tex/conclusion.tex <==
We have improved the upper bound on provability for 
the broad class of
axiomatic extensions of 
$\mathbf{FL_{ec}}$ and
$\mathbf{FL_{ew}}$ by acyclic $\mathcal{P}_3$-axioms, or, equivalently, for all axiomatic extensions of these logics captured by
analytic hypersequent structural rules.
In particular, we improved the upper bound for the complexity of $\mathbf{MTL}$.

These results are surprising
because they break the expectation that
hypersequent calculi cause an expressive `$\omega$-jump'
in complexity when compared to sequent calculi.
In the case of contraction, we obtained optimality:
if tighter bounds are to be sought, the class of logics
being covered must be restricted (to ones that exclude
$\mathbf{FL_{ec}}$).
In the case of weakening, the possibility of 
getting better bounds for the whole class is still open,
since, as far as we know, no logic in this class is known
to be hard for Ackermann ($\mathbf{FL_{ew}}$, for example, is PSPACE-complete). 
There have been many successful cases
in the literature where algorithms based on Dickson's lemma had their complexity reduced by a finer analysis
on the length of the produced bad sequences~\cite{LazicS16,LazicS21}. Our
algorithm provides a good starting framework towards better bounds
via such approaches.


 
